Lost in Tracking: Uncertainty-guided Cardiac Cine MRI Segmentation at Right Ventricle Base

Accurate biventricular segmentation of cardiac magnetic resonance (CMR) cine images is essential for the clinical evaluation of heart function. However, compared to left ventricle (LV), right ventricle (RV) segmentation is still more challenging and less reproducible. Degenerate performance frequently occurs at the RV base, where the in-plane anatomical structures are complex (with atria, valve, and aorta) and vary due to the strong interplanar motion. In this work, we propose to address the currently unsolved issues in CMR segmentation, specifically at the RV base, with two strategies: first, we complemented the public resource by reannotating the RV base in the ACDC dataset, with refined delineation of the right ventricle outflow tract (RVOT), under the guidance of an expert cardiologist. Second, we proposed a novel dual encoder U-Net architecture that leverages temporal incoherence to inform the segmentation when interplanar motions occur. The inter-planar motion is characterized by loss-of-tracking, via Bayesian uncertainty of a motion-tracking model. Our experiments showed that our method significantly improved RV base segmentation taking into account temporal incoherence. Furthermore, we investigated the reproducibility of deep learning-based segmentation and showed that the combination of consistent annotation and loss of tracking could enhance the reproducibility of RV segmentation, potentially facilitating a large number of clinical studies focusing on RV.

==> tables/table2_reproduce.tex <==
% \begin{table}[htb]
% % \setlength\extrarowheight{5pt}
% \small
% \caption{Mean and standard deviation of volumetric prediction reproducibility $\sigma_v$ [mL] on the test set derived from Bayesian ensembles.}
% \label{table:reproduce}
% \centering
% \begin{tabular}{p{3cm}<{\centering}p{3cm}<{\centering}p{3cm}<{\centering}}
% \toprule
% % \midrule
% \textbf{Variants} & \textbf{ED} & \textbf{ES} \\
% \midrule
% Original, U-Net & 4.9±5.2 & 3.6±3.8 \\
% New, U-Net & 4.8±7.0& 3.0±2.7\\
% New, Proposed & 4.1±2.9 & 3.0±1.7 \\
% \bottomrule
% \end{tabular}
% \end{table}

